On Information Asymmetry in Competitive Multi-Agent Reinforcement Learning: Convergence and Optimality

In this work, we study the system of interacting non-cooperative two Q-learning agents, where one agent has the privilege of observing the other's actions. We show that this information asymmetry can lead to a stable outcome of population learning, which generally does not occur in an environment of general independent learners. The resulting post-learning policies are almost optimal in the underlying game sense, i.e., they form a Nash equilibrium. Furthermore, we propose in this work a Q-learning algorithm, requiring predictive observation of two subsequent opponent's actions, yielding an optimal strategy given that the latter applies a stationary strategy, and discuss the existence of the Nash equilibrium in the underlying information asymmetrical game.

==> big_tau.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=4.3in,
%at={(0.745in,0.481in)},
at={(0.5in,0in)},
scale only axis,
xmin=0,
xmax=50,
xlabel style={font=\color{white!15!black}},
xlabel={iteration k},
ymin=1,
ymax=4,
ylabel style={font=\color{white!15!black}},
%ylabel={Value V},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
%legend style={at={(0.97,0.03)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, line width=1.5pt]
  table[row sep=crcr]{%
0	0.777322076016123\\
1	1.40084701792734\\
2	1.89110207162868\\
3	2.27744387090406\\
4	2.58734262836391\\
5	2.83462039296388\\
6	3.03329261231975\\
7	3.18978846344124\\
8	3.31685401549246\\
9	3.41809547615989\\
10	3.49941891477444\\
11	3.56421756453625\\
12	3.61642878554034\\
13	3.65843677723074\\
14	3.69206775443376\\
15	3.71869362350256\\
16	3.73989680186737\\
17	3.75684283792428\\
18	3.77056772004311\\
19	3.78152124188325\\
20	3.79029592941398\\
21	3.79725832039782\\
22	3.80274802316739\\
23	3.8072343626697\\
24	3.81082538256956\\
25	3.81370659703922\\
26	3.81602827396496\\
27	3.81785498818976\\
28	3.81933205641387\\
29	3.82050448811849\\
30	3.82144933069852\\
31	3.8221969755449\\
32	3.82279454565761\\
33	3.82327693920612\\
34	3.82366460886991\\
35	3.82397334074095\\
36	3.82421932597909\\
37	3.8244138612932\\
38	3.82457033226242\\
39	3.82469583816551\\
40	3.82479697306821\\
41	3.82487743247949\\
42	3.82494125208128\\
43	3.82499281247686\\
44	3.82503385918313\\
45	3.82506669105286\\
46	3.82509317205777\\
47	3.82511447158683\\
48	3.82513151121007\\
49	3.82514493413755\\
};
%\addlegendentry{Greedy and Greedy}

\addplot [color=mycolor2, dotted, line width=1.5pt]
  table[row sep=crcr]{%
0	0.745831905454641\\
1	1.33089716218409\\
2	1.79578074886012\\
3	2.16011535264162\\
4	2.45389744256102\\
5	2.68735029692985\\
6	2.87524336733526\\
7	3.0257726571804\\
8	3.14730897586426\\
9	3.24363791644108\\
10	3.32050016320093\\
11	3.3819903920422\\
12	3.43169706218229\\
13	3.47120768890171\\
14	3.50219543817577\\
15	3.52707933640169\\
16	3.54712589708508\\
17	3.56311041821024\\
18	3.57593112705141\\
19	3.58624216322239\\
20	3.59458642379313\\
21	3.60117625689036\\
22	3.60637868634326\\
23	3.61059697411903\\
24	3.61399941531876\\
25	3.61671929780977\\
26	3.61887434072093\\
27	3.62060196215064\\
28	3.62198374675671\\
29	3.62309203224028\\
30	3.62397939324419\\
31	3.62468449059425\\
32	3.62525257567971\\
33	3.62570378979432\\
34	3.62606656685597\\
35	3.62635576782247\\
36	3.62658865463457\\
37	3.62677369974045\\
38	3.62692188201442\\
39	3.62704259559862\\
40	3.627137417552\\
41	3.62721430315688\\
42	3.62727633984716\\
43	3.62732563451235\\
44	3.62736484092326\\
45	3.62739659393807\\
46	3.62742165907677\\
47	3.62744194224823\\
48	3.62745791441245\\
49	3.62747064977141\\
};
%\addlegendentry{Boltzman and Greedy}

\addplot [color=mycolor3, dashed, line width=1.5pt]
  table[row sep=crcr]{%
0	0.634006926747742\\
1	1.14209313977263\\
2	1.53097744305491\\
3	1.84563465465995\\
4	2.08937654061607\\
5	2.28993092684305\\
6	2.44717640002433\\
7	2.57442768271176\\
8	2.67847525111006\\
9	2.76041114523034\\
10	2.8259467891516\\
11	2.87730843622909\\
12	2.91980005062108\\
13	2.95267327105674\\
14	2.97975756279544\\
15	3.00106792040713\\
16	3.01837046400057\\
17	3.03204417968483\\
18	3.04303456365608\\
19	3.05184627127625\\
20	3.05893664704192\\
21	3.06459170501495\\
22	3.06906641573191\\
23	3.07263419484614\\
24	3.07552556729615\\
25	3.07784295090634\\
26	3.07967978389868\\
27	3.08115888472511\\
28	3.08231568364834\\
29	3.08326493600781\\
30	3.08401376344881\\
31	3.0846134790706\\
32	3.08509506914085\\
33	3.08547919935403\\
34	3.08579211024336\\
35	3.08604198691611\\
36	3.0862403949275\\
37	3.08639945902706\\
38	3.08652562704554\\
39	3.08662677696146\\
40	3.08670793813792\\
41	3.08677285432993\\
42	3.08682516952721\\
43	3.0868666122186\\
44	3.08689950893953\\
45	3.08692625334665\\
46	3.08694813648327\\
47	3.08696529396326\\
48	3.08697902432514\\
49	3.08698987972338\\
};
%\addlegendentry{Greedy and Boltzman}

\addplot [color=mycolor4, dashdotted, line width=1.5pt]
  table[row sep=crcr]{%
0	0.541482828536854\\
1	0.97450788672798\\
2	1.31461677309335\\
3	1.59172993072559\\
4	1.81027306636771\\
5	1.99019956396973\\
6	2.12809790484256\\
7	2.23751410971901\\
8	2.32723900415227\\
9	2.40006040941123\\
10	2.45710543386389\\
11	2.50262594530019\\
12	2.53876384155771\\
13	2.56815974942115\\
14	2.59171802919617\\
15	2.61033324918401\\
16	2.62576459431515\\
17	2.63803712186151\\
18	2.64770918108958\\
19	2.65547766083448\\
20	2.66166700043248\\
21	2.6666226410702\\
22	2.67064264638552\\
23	2.67382930269402\\
24	2.67635591146023\\
25	2.67839398634763\\
26	2.67999074821577\\
27	2.68129259952641\\
28	2.68230284087827\\
29	2.68311562724396\\
30	2.68377503954183\\
31	2.68429483128745\\
32	2.68471812619363\\
33	2.68506020640047\\
34	2.68533223361885\\
35	2.68554690779732\\
36	2.68571834680534\\
37	2.68585808129521\\
38	2.68597159684746\\
39	2.68605872010716\\
40	2.68613007297248\\
41	2.68618594859517\\
42	2.68623066525444\\
43	2.68626711757696\\
44	2.68629609380172\\
45	2.68631966934286\\
46	2.68633831066827\\
47	2.68635353533323\\
48	2.68636559456309\\
49	2.68637501603108\\
};
%\addlegendentry{Boltzman and Boltzman}

\end{axis}

\begin{axis}[%
width=5.729in,
height=4.375in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\end{axis}
\end{tikzpicture}%
